SDSS IV MaNGA: Visual Morphological and Statistical Characterization of the DR15 sample

We present a detailed visual morphological classification for the 4614 MaNGA galaxies in SDSS Data Release 15, using image mosaics generated from a combination of r-band (SDSS and deeper DESI Legacy Surveys) images and their digital post-processing. We distinguish 13 Hubble types and identify the presence of bars and bright tidal debris. After correcting the MaNGA sample for volume completeness, we calculate the morphological fractions, the bi-variate distribution of type and stellar mass M*-where we recognise a morphological transition "valley" around S0a-Sa types- and the variations of the g-i colour and luminosity-weighted age over this distribution. We identified bars in 46.8% of galaxies, present in all Hubble types later than S0. This fraction amounts to a factor ~2 larger when compared with other works for samples in common. We detected 14% of galaxies with tidal features, with the fraction changing with M* and morphology. For 355 galaxies, the classification was uncertain; they are visually faint, mostly of low/intermediate masses, low concentrations, and disky in nature. Our morphological classification agrees well with other works for samples in common, though some particular differences emerge, showing that our image procedures allow us to identify a wealth of added value information as compared to SDSS-based previous estimates. Based on our classification, we also propose an alternative criteria for the E-S0 separation, in the structural semi-major to semi-minor axis versus bulge to total light ratio (b/a-B/T) and concentration versus semi-major to semi-minor axis (C-b/a) space.

==> extra.tex <==






%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Numeros calculados en el draft

\subsection{Morphology and Structure in the Star Formation Main Sequence Diagram}
 
Calculando las fracciones sin edge-on son (total=2963):
starbusrt: 13.9
starform: 20.3
green v:  45.2
red seq: 8.1
abajo de ls RS: 12.4



Toñito: calcular que  valores de B/T representativos de MaNGA y con que %  en las cuatro familias Starbursts, main squence, green valley y red sequence (quitando las inclinadas)
porcentaje disk-dominated /MaNGA   21.9
porcentaje intermedias /MaNGA   48.1    
porcentaje bulge-dominted /MaNGA   30.0


\subsection{Bars and AGNs}

Toñito: Puedes guardar estos resultados en algun archivo
Seria bueno ir guardando tambien todos los resultados numericos de las otras secciones. Cuando los hayas guardado todos me dices y los voy borrando



Resultados Bars-AGN
OJO Toñito: quitar las Es de la estadistica
Numero de Bars + AGNs:  34
Numero de no-Bars + AGNs: 41 (no E)
Toñito: te pareceria agrupar strong bars como (B y AB_) 
y las weak bars como (AB y A_B)
Numero de strong Bars (B y AB_) + AGNs:27
Numero de weak Bars (AB y A_B) + AGNs:7
Numero de strong Bars (B y AB_) + AGNs tipo I: 11
Numero de strong Bars (B y AB_) + AGNs tipo II: 16


Numero de weak Bars (AB y A_B) + AGNs tipo I: 1
Numero de weak Bars (AB y A_B) + AGNs tipo II: 6

\subsection{AGNs and Tidal Features}


AGNs + tides:16
no-AGNs + tides: 721
AGN I + tides: 6
AGN II + tides: 10

 



%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{AGN and bars }

Figuras hechas buscando una relacion entre agn y  bars

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/barAGN_class.png}
 \caption{number of AGNs, with bar and without bar }
 \label{}
\end{figure}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/barAGN_col_mass.png}
 \caption{AGN histogram in function of colour and mass, divided by B and AB families, normalised to the total number of AGNs}
 \label{}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{MorphoClass}

Figure~\ref{fig:ES0S0a_mosaic1} shows representative examples of early type E (two upper panels), S0 (two intermediate panels) and S0a (two lower panels) MaNGA galaxies. Each pair of panels, show the SDSS images (above) followed by the corresponding DESI legacy images (below). Similar to that shown in Figure~\ref{fig:mosaic}, along each panel, 
and from left to right, a gray logarithmic-scaled r-band image, a filter-enhanced r-band image and a $gri$/$grz$ color image are shown. 

Notice the gradual appearance of disky features (sharp edges and possible spiral arms) when going from E's to S0s and transition S0a galaxies.
 
 
\begin{figure}
\includegraphics[width=\columnwidth]{figures/manga-early-mos-paper.png}
 \caption{E, S0 and S0a MaNGA galaxies. Two upper panels: The E-type galaxy manga-7958-1901 From left to right; SDSS gray logarithmic-scaled r-band image, filter-enhanced r-band image and $gri$ color image, followed below by the corresponding DESI legacy images. Two Middle panels: The S0-type galaxy manga-7968-9102. Two bottom panels: The S0a-type manga-8451-6102}
 \label{fig:ES0S0a_mosaic1}
\end{figure}


Figure~\ref{fig:Sa-Irr_mosaic} is a mosaic containing four pairs of horizontal panels (from top to bottom). Each pair of panels illustrates our combination of images from SDSS (above), DESI (below) and its corresponding filter enhanced image. Notice the gradual change in morphological types depending on the prominence of the bulge, tightness of the arms, and the degree of resolution of structure along the arms/outer disk, up to Irr types (bottom pair of panels) where the spiral structure disappear. The presence/absence of a bar was confirmed (SB), or suspected (SAB) in other cases. Notice also the contribution in morphological details that the DESI legacy images provide in the outskirts.
 

\begin{figure*}
 \includegraphics[width=2\columnwidth]{figures/manga-late-mos-paper.png}
 \caption{Sa-Irr galaxies. A mosaic showing four pairs of horizontal panels (from top pair to bottom pair). Each pair shows from left to right; a SDSS/DESI gray logarithmic-scaled r-band image, a filter-enhanced r-band image and the corresponding $gri$/$grz$ color image.  Top pair of panels: manga-7815-6103, Intermediate upper panel: manga-8992-12704, Intermediate lower panel: manga-8948-12703, Bottom pair of panels: manga-8443-12701).}
 \label{fig:Sa-Irr_mosaic}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%FIGURE%%%%%%%%%%%%%%%
\begin{figure*}
%trim=l b r t
\centering
\includegraphics[trim = 3mm 67mm 31mm 0mm, clip, width=\textwidth]{figures/GSMF_weighted}
\caption{Galaxy Stellar Mass Function.  \textit{Left Panel:} NSA GSMF is presented as black empty circles with errorbars, orange shaded regions is the non-corrected MaNGA GSMF. In black solid line, we plot the MaNGA GSMF taking into account volume corrections. \textit{Right Panel:} GSMF decomposed in contributions from different morphological types, this inferences are taking into account volume completeness corrections determined in Calette et al. (in prep). Morphological types are color coded as presented at the top right corner of the panel.} 
\label{fig:GSMFs-morphs} 
\end{figure*}
%%%%%%%%%%%%% END FIGURE%%%%%%%%%%%%%


\section{Stellar mass function}
%{\color{red}Aldo: Ruben puedes encargarte de esta seccion}\\
We calculate volume corrections for the MaNGA sample following the methodology presented above. We use such corrections to calculate the GSMF of all MaNGA galaxies and GSMFs for each galaxy morphology considered in this work (see section 3 for details). In figure \ref{fig:GSMFs-morphs} we present such results. First, on the left panel we plot the GSMF inferred from MaNGA as if it were a complete sample in stellar mass with orange shaded regions, the GSMF appliying


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/CAS_BT_sfr.png}
 \caption{CAS vs BT, sfr}
 \label{fig:CAS_BT_sfr}
\end{figure}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/mass_ssfr.png}
 \caption{Mass vs sfr by morphological type}
 \label{fig:mass_sfr}
\end{figure}


\section{Comparing with a CNN morphological classification}



\textcolor{cyan}{Given that \citetalias{Fischer2019} present the Deep Learning TType morphology (trained using the \citealt{Nair2010} catalogue) and the photometric parameters for the MaNGA (DR15) galaxies, we can compare straightforward our morphological results in terms of their classification and using also their photometric parameters.}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/class_DS18col.png}
 \caption{One to one comparison with \citetalias{Fischer2019} morphology}
 \label{fig:class_comp}
\end{figure}

\textcolor{cyan}{Figure~\ref{fig:class_comp} shows the comparison between our classification and \citetalias{Fischer2019} ML classification. Colour bar defines the number density per bin. Even though the apparent large scatter, our classification are in good agreement for Ellipticals and intermediate Late types galaxies. This can also be seen in Figure~\ref{fig:hist_class_comp}, where differences between the two classifications are presented ($\Delta$TType). These histograms also show considerable differences for our S0, S0a and Sa types. One of the possible reasons is definitively the method we are using to distinguish among these galaxies. Back to Figure~\ref{fig:ES0S0a_mosaic2}, we demonstrated how galaxies can easily be confused, specially when only SDSS are seen. Then, many galaxies that were considered as Ellipticals by \citetalias{Fischer2019} are in reality later types, for instance.}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/hist_comp_class.png}
 \caption{$\Delta$TType (Ttype $-$ Ttype$_{DS18}$ ) classification histogram comparing with \citetalias{Fischer2019}}
 \label{fig:hist_class_comp}
\end{figure}



\textcolor{cyan}{Figure~\ref{fig:hist_serc_comp} shows the S\'ersic index corresponding to the best fit, either a single S\'ersic or a double S\'ersic component fit (taking into account the $flipped$ galaxies), according to the flags described in \citetalias{Fischer2019}, following the same morphological and colour code separation, E (magenta), S0 (orange), early Late type (0 $<$ TType $<$ 3; green) and very Late type (0 $<$ TType $<$ 3; blue) galaxies.} 

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/hist_sercB_class.png}
 \caption{S\'ersic index histogram by morphological type comparing with \citetalias{Fischer2019}}
 \label{fig:hist_serc_comp}
\end{figure}



Esta seccion es tambien de comparacion con CNN

\subsection{Morphological Content and Structural Parameters}

We put our morphological evaluation on a parametric basis by retrieving photometric parameters from 
S\'ersic and S\'ersic + Exponential fits to the 2D surface brightness profiles of the MaNGA Data Release 
15 (DR15) galaxy sample after a re-analysis and homogeneization by \citetalias{Fischer2019} in a PyMorph Photometric Value Added Catalogue (MPP-VAC) \footnote{The MPP-VAC is one of the value added catalogues of the SDSS DR15 release and is available on line: www.sdss.org/dr15/data access/value-added-catalogs/manga-pymorph-d
r15-photometric-catalog}.  Tonito: Explicar el detalle de como (con que criterios) se seleccionaron estos parametros...

We use the set of parameters measured in the SDSS r band and follow the flag system implemented for the MPP-VAC catalogue. We also adopt their refitting and/or flipping. First we avoid the flags FLAG_FAILED_S and FLAG_FAILED_SE set to 1 or 3 meaning that they have a failed S\'ersic or SerExp fit or both, respectively. There is a preference system given by FLAT_FIT. FLAG FIT=1
indicate that the parameters from the single-S\'ersic fit are preferred. FLAG FIT=2 is always supported
by the goodness of fit \chi^2 for the two-component SerExp fit. In some cases, the two models are acceptable for the two- and single-component fits, respectively, so FLAG FIT=0. 

Antes que otra cosa hay que entender bien como se estimaron los parametros estructurales en el 
trabajo de Fischer y que flags sugiere utilizar:

Aqui te escribo algunas consideraciones para comparar con los tipos morfologicos de Fischer:

They mainly use the TType and PS0
to define two classes of LTGs:
those with TType>3, and others with 0<TType<3; objects having
TType<0 andPS0 ≥0.5 are defined to be S0; and ellipticals (E) have
TType < 0 and PS0 < 0.5.

Para comparar lenticulares contra nosotros y separarlas de las Early-spirals:
Ver fig. 12 in DS18 shows
that while TType=0 is a reasonable choice for separating S0s from
other LTGs, the actual boundary is not particularly sharp. By setting
the threshold at TType=0, objects we classify as LTGs may be
contaminated by S0s, more than vice versa. OJO: Habra que discutir esto con detalle.

Para el parametro: ε = 1 − b/a.
For objects having FLAG FIT = 0 or FLAG FIT = 2, the quantity
b/a is the semiminor/semimajor axis ratio of the total SerExp fit (i.e.
BA_SE in Table 1.


a TType value, a finer separation between
S0 and pure ellipticals (E), and the probability of having a
bar feature. Pedge-on is the probability that a
galaxy is edge-on, there is also Pbar, Pbulge, and Pcigar. Since the models return probabilities, a user-defined threshold
value (Pthr) can be used to select objects of a certain type. Ojo values of precision (∼ purity) and True Positive Rate (TPR ∼ completeness) for three Pthr values are tabulated in table 2 of DS18.

The typical error in TType is ∼1.1
PS0 (which is only meaningful for
‘early-type’ galaxies, ETGs, i.e. when TType ≤ 0).
OJO: A flag is provided for the TType (flag TT) and PS0 (flag S0), indicating when the original output
of the model has been changed after visual inspection.

Pmerg value is a good indicator of projected
pairs or nearby objects rather than of real ongoing mergers. We
found it extremely useful for identifying galaxies whose MaNGA
spectroscopic data were contaminated by neighbours.We find that∼
50 per cent of the galaxies with a contaminated spectrum have Pmerg
> 0.5, compared to ∼ 17 per cent for the whole sample. Increasing
the limit, only ∼ 11 per cent of the whole sample has Pmerg > 0.8,
while this fraction is ∼ 40 per cent for the contaminated sample.

Una posible ruta de seleccion: 
1. FLAG FIT =/ 3
2. flaggs as having two components, one component, or
for which both descriptions are equally acceptable.


 

A first view of the relationship among structural parameters and morphology of galaxies in the 
MaNGA sample is presented. We start by showing in Figure~\ref{fig:hist_serc} the S\'ersic index distribution (Tono: Cual Sersic? with FLAG FIT =1 o 2?)  in terms of our classification in four main bins. As expected late type galaxies shows low $n$ values and ellipticals tend to have a maximum between $n$ 5 and 6. Nevertheless, S0 galaxies show a flat distribution between $n$ 1 and 6.
Tono: Yo sugiero que todas estas figuras lleven fraccion en el eje y para poder comparar mas adelante vs Fischer.




\begin{figure}
 \includegraphics[width=\columnwidth]{figures/ssfr_class2D.png}
 \caption{2D histogram (same as Figure~\ref{fig:mass_morpho2D}) for Hubble type and sSFR \textcolor{red}{CORREGIDA!}}
 \label{fig:mass_morpho2D}
\end{figure}



 quitar++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
\subsection{Bars and AGNs}

The relation between stellar bars (typically identified at optical wavelengths) and the presence of an AGN (also identified by optical line ratios or equivalent widths) in galaxies has been a matter of intense debate in the last years. In more recent years the advent of big extragalactic surveys have provided unprecedented statistical significance to these studies but still no conclusive results has been forcefully established either confirming or ruling out such correlations. 

This situation may change in the forthcoming years thanks to the advent of recent IFU surveys in nearby galaxies like CALIFA (), MaNGA () and MUSE () providing (i)  detailed spatially resolved information with (ii) higher spectroscopic resolution in (iii) statistically significant samples, very valuable to re-examine the relationship between bars and AGNs in nearby disc galaxies.

Here we bring together various results of our homogeneous morphological characterization of the MaNGA sample with the identification AGNs, after an AGN classification scheme by \citet{Sanchez2018} (see section ()) to explore the relation of stellar bars and AGNs in the MaNGA sample. We consider the physical scenario for the incidence of AGNs given the presence of bars (and bar families) in the MaNGA sample.

A first direct result (with no match in stellar mass and color), is that the fraction of barred galaxies with AGNs (45\%) is lower than the fraction of non-bared galaxies with AGNs (55\%). However we look more closely for any relationships between our detailed identification of stellar bars and their bar families (section ()) and AGN types (I and II). 

Figure~\ref{fig:bar-agn} shows in the upper panel (left), the morphological distribution of galaxies that simultaneously host a stellar bar and a AGN (bar+AGN; dot-dashed red line), compared to the distribution for non-barred galaxies that host an AGN (non-bar+AGN; black solid line). Similarly, the upper  panel (right) shows the corresponding stellar mass distribution. In both panels, additional colored histograms identify strong bars (AB\_+B) with AGNs (yellow) and weak bars (\_AB+AB) with AGNs (pink). The lower panel show the same distributions but this time with additional colored histograms identifying 
weak bars + type I AGNs (purple deep), strong bars + type I AGNs (crossed lines),
strong bars + type II AGNs (pink) and weak bars + type II AGNs (soft blue).
Notice that in both barred and non-barred samples, only disk galaxies were 
considered.
{\color{red} revisar las ultimas lineas}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/barAGN_morp_mass.png}
 \caption{Top: Bar+AGN (dashed-red) and non-bar+AGN (black line) distributions as a function of Hubble type (left) and stellar mass (right), normalised to the total number in each sample. Weak (strong) bars are coloured in red (yellow). Bottom: Same distributions including either weak and strong bars as well as type I and II AGNs. Notice that in both barred and non-barred samples, only disk galaxies were considered. {\color{red} REVISADA}}
 \label{fig:bar-agn}
\end{figure}

While non-barred disk galaxies with AGNs are distributed from S0 to Sbc types, with most of them in early (S0 - Sab) types (85\%), barred disk galaxies with AGNs are distributed from Sa to Sc types, with most of them in intermediate/late (Sb - Sc) types (73\%).  

Weak bars with AGNs are located only in intermediate/late (Sb - Sc) types, contributing to a small fraction (20.6\%) of all barred galaxies with AGNs. In contrast, strong bars with AGNs are broadly distributed and with a dominant fraction (79.4\%).  

Barred galaxies with AGNs are slightly skewed towards higher stellar masses 
(median logM* =10.5) than non-bared galaxies with AGNs (median logM* =10.42) but the difference is not significant (Kruskal-Wallis test p =0.12 ). Notice also a wider mass distribution of strong barred galaxies with AGNs (median logM* =10.49) compared to weak barred galaxies with AGNs that show a narrow mass distribution but a slightly larger value (median logM* =10.58). However, these differences are not significant (Kruskal-Wallis test p =0.48)
 
In addition to the morphological (left panel) and Mass distributions (right panel), the lower panel of Figure~\ref{fig:bar-agn} shows the distributions of barred galaxies with type I and II AGNs. Barred galaxies show a similar morphological distribution whether hosting type I or II AGNs 
but with a dominant fraction of type II AGNs (65\%) compared to type I AGNs (35\%). Barred galaxies that host type I AGNs are preferently found in the high mass extreme of its distribution (median logM= 10.64), compared to barred galaxies hosting type II AGNs that show a more wide distribution (median logM=10.48 ). However, these differences are not significant (Kruskal-Wallis test p =0.39)  

Resultados Bars-AGN
OJO Toñito: quitar las Es de la estadistica
Numero de Bars + AGNs:  34
Numero de no-Bars + AGNs: 41 (no E)
Toñito: te pareceria agrupar strong bars como (B y AB_) 
y las weak bars como (AB y A_B)
Numero de strong Bars (B y AB_) + AGNs:27
Numero de weak Bars (AB y A_B) + AGNs:7
Numero de strong Bars (B y AB_) + AGNs tipo I: 11
Numero de strong Bars (B y AB_) + AGNs tipo II: 16

Numero de weak Bars (AB y A_B) + AGNs tipo I: 1
Numero de weak Bars (AB y A_B) + AGNs tipo II: 6

Strong barred galaxies with AGNs (\%) are a factor of 4 more frequent than weak bars with AGNs (\%) in the MaNGA sample.
However, we caution the reader that this may be reflecting our difficulty to detect weak bars in our visual inspection inspite of the combination of images and processing used here. Various aspects may be influencing these results, like image resolution, the observation band and the range of redshifts covered by the MaNGA sample. These results may also be reflecting our inhability to detect weak AGNs as already emphasized from the optical nature of their selection in the MaNGA sample.
Our preliminary results are consistent with no relationship of the presence of an AGN given a large-scale galactic bar in the MaNGA sample.



\subsection{AGNs and Tidal Features}

It is important to recognize two main components on the issue of the merger-AGN connection. The first is whether mergers can trigger AGN and the second is whether mergers are the dominant AGN trigger. To the first question the answer appears positively established, at least at low z (c.f. \citealt{Ellison2019} and reference therein). To the second question, there seems to be no clear concensus or definite conclusions. On one side some studies (Gabor et al. 2009; Cisternas et al. 2011; Kocevski et al. 2012; Mechtley et al. 2016) and simulations (Draper \& Ballantyne 2012; Bellovary et al. 2013; Menci et al. 2014; Steinborn et al.
2018) conclude that mergers can contribute but are not the dominant fuelling pathways of AGNs.

However, as argued by \citet{Ellison2019}, before stating a conclusion, care must be taken when synthesizing the results from studies using different AGN selection techniques, in different luminosity regimes and also at different redshifts. Selecting AGN with different techniques leads to AGN (and host galaxies) with different properties (e.g. Hickox et al. 2009; Best & Heckman 2012; Mendez et al. 2013; Gurkan et al. 2014; Ellison et al. 2016). The impact
of selecting AGN at different wavelengths on the interpretation of
the merger-AGN connection has been clearly demonstrated by Satyapal et al. (2014), who showed that mergers show a greater excess of mid-IR selected AGN, compared with AGN that are selected on the basis of their optical emission lines. Whilst both mid-IR selected and (to a lesser extent) optically selected AGN are more common in mergers than in isolated galaxies, z ∼ 0 low excitation radio galaxies appear to be secularly triggered \citep{Ellison2015}. The issue of a ‘merger-AGN connection’ therefore depends critically how
one defines ‘AGN’.

As stated in Sections () and () we use an optically selected MaNGA AGN sample, 
carefully selected by using the crteria established in Sanchez te al. 2018 and cross-correlate it with the MaNGA sample where we have detected tidal features  using deep r-band imaging from the DESI legacy survey. With both information at hand, we estimate the frequency of morphologically disturbed galaxies in the MaNGA AGN sample.

Toñito: Vamos a hacer lo siguiente:
Queremos responder la pregunta: whether mergers are the dominant AGN trigger.

Otra vez no me queda claro si deben hacerse como en numero N en cada bin o como fraccion dividiendo por el numero total en cada bin??

1. Hacemos un histograma de todos los AGNs + Tides por tipo morfologico 
y  un histograma de todos los no-AGNs + Tides en el mismo plot y
lo comparamos ahi mismo marcamos con color los histogramas de  AGNs tipo I y II.
2. Hacemos un histograma de todos los AGNs + Tides por masa estelar 
y  un histograma de todos los no-AGNs + Tides en el mismo plot y
lo comparamos ahi mismo marcamos con color los histogramas de  AGNs tipo I y II.

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/tideAGN_morp_mass.png}
 \caption{Tides+AGNs (dashed-red) and tides+nonAGNs (black) distributions as a function of Hubble type (left) and stellar mass (right), normalised to the total number of galaxies in each sample (16 and 721). Type I (type II) AGNs are presented in red (yellow) coloured bars. {\color{red} REVISADA}}
 \label{fig:tides-agn}
\end{figure}


AGNs + tides:16
no-AGNs + tides: 721
AGN I + tides: 6
AGN II + tides: 10

 

y vemos que resultados obtenemos.

OJO Esto para AGN-Tides:
The fact that galaxies
in low density groups, strongly affected by tidal in-
teractions and with signatures of E+A spectra, are
more frequently found in the GV (e.g. Bitsakis et al.
2016) supports the scenario that these are galaxies
undergoing transformation.

quitar hasta aqui++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++


\section{Volume-Correction}

%To this purpose we use as a reference the $NSA$ sample \cite{Blanton+2017} such that from that sample we will be selecting $K$-corrected magnitudes at $z=0$, stellar masses, $M_{\ast}$, galaxy colors, $g-r$, and redshifts for the MaNGA sample. An empirical model for the E-correction at $z=0$ described in \cite{Dragomir+2018} will also be included. 


%For a volume-limited sample that is complete in stellar mass, the simplest estimator for the GSMF is given by $\phi_{\ast}(M_{\ast})d\log M_{\ast}=N_{g}(M_{\ast})/V$, where $N_{g}$ is the number of galaxies at the mass range $\log M_{\ast}\pm d\log M_{\ast}/2$ and $V$ is the co-moving volume of the sample. Here, we use the above estimator to estimate the expected fraction of galaxies, $f_m$, as a function of stellar mass, color and redshift for the MaNGA sample. As shown in \citep[][see also \citet{Rodriguez-Puebla+2020}]{Sanchez+2019}, the 



%The above estimator provides the expected number of galaxies with stellar masses between $\log M_{\ast}\pm d\log M_{\ast}/2$ in a redshift range $z\pm dz/2$ as $\left\langle N_g(M_{\ast},z)\right\rangle$ = $\phi_{\ast}d\log M_{\ast}/dV(z)$. If $\left\langle N_M(M_{\ast},z)\right\rangle$ is the expected number of galaxies in the MaNGA sample over the same stellar mass and redshift range then $f_m(M_{\ast},z)=\left\langle N_M(M_{\ast},z)\right\rangle/\left\langle N_g(M_{\ast},z)\right\rangle$. Equivalently, $f_m(M_\ast,z)=\left\langle \phi_{M,\ast}(M_\ast)\right\rangle/ \phi_{\ast}(M_\ast)$, where $\left\langle \phi_{M,\ast}(M_\ast)\right\rangle$ is the average uncorrected GSMF from MaNGA. Thus, we compute $\left\langle \phi_M(M_{\ast})\right\rangle$ as

%\begin{equation}
%    \left\langle \phi_M(M_{\ast})\right\rangle = \sum_{i}^{N_z}\phi_{M,i}(M_\ast,z_i)\times w_i,
%\end{equation}

%where $\phi_{M,i}(M_\ast,z_i)d\log M_\ast=N_{M,i}(M_\ast,z_i)/dV(z_i)$ with $N_{M,i}(M_\ast,z_i)$ as the real observed number of galaxies in MaNGA with stellar masses $\log M_\ast\pm d\log M_\ast$ at $z_i\pm dz/2$. Weights, $w_i$, are defined as $w_i=N_{M,i/\sum_i N_{M,i}}$. Summation over $i$ refers to redshift and $\sum w_i=1$. Thus, the expected number of galaxies complete in stellar mass based on MaNGA is $N_{M,V}(M_\ast,z_i)/f_m(M_\ast,z)$.

%In principle, stellar-mass bins and redshift bins can be defined as small as we want in order to have $N_M(M_\ast, z_i)=1,0$ objects per bin. Thus for the \textit{j}th galaxy in the sample with stellar mass $M_\ast$ and redshift $z$ the volume correction is given by 
%\begin{equation}
%   \frac{1}{V_j}=  \frac{w_i(M_\ast, z)}{f_m(M_\ast, z)dV (z)} .
%\end{equation}

%In practice it is not required that $N_M(M_\ast, z_i)=1,0$ objects per $M_\ast$ and $z$ bin since the resulting volume corrections would be dominated by Poisson noise due to the low number of galaxies in MaNGA.
%Instead, we calculate an average volume correction $1/V$  by creating a grid of 30 redshift bins within $0.03<z<0.17$ and 50 stellar mass bins within $10^8 < M_\ast/M_\odot < 10^12$. Thus for every galaxy
%with $M_\ast$ and redshift $z$ we use cubic spline interpolations to find its corresponding volume correction from a grid of $1/V_{i,j}$ over the \textit{i}th stellar-mass bin and the \textit{j}th redshift bin. In the general case in which $f_m$ also depends on galaxy colours, the above procedure is still valid.  


%As a result of this volume correction, every galaxy has a weight associated ($w_i$). When counting galaxies, without considering any weight, every galaxy count 1; however, if we want to apply the volume correction in our counting, every galaxy must be multiplied by its $w_i$, in other words, we are counting the $w$'s. Then the total weighted sum will be

%\begin{equation}
%\label{eq:weight}
%    N_w = \sum_{i}^{N} w_i \times 1 .
%\end{equation}


\section{structural parameters}

\textcolor{cyan}{Similar to Figure 22 in \citetalias{Fischer2019} and following the same morphological and colour code separation (E, magenta; S0, orange; early Late type 0 $<$ TType $<$ 3, green; and very Late type 3 $\leq$ TType , blue), Figure~\ref{fig:hist_BT_comp} shows the B/T distribution as a function of our morphology {\color{red}and  \citetalias{Fischer2019} morphology (right panel). Very late type galaxies shows a similar distribution, dominating at low B/T values in both cases, as expected; intermediate types also are similar, except that, our distribution has a longer tail of B/T values towards 1, probably reflecting the higher number reported for Sa type. For S0 and E, our distributions tend to be flat over the range of 0.3-0.9, with slightly maximums around 0.85, meanwhile for \citetalias{Fischer2019} are more concentrated with maximums at $\sim$0.5 and $\sim$0.85 respectively; although of these differences, it is clear early type galaxies tend to have light more concentrated and then higher B/T values. If the B/T parameter were estimated using the DESI Legacy survey (with deeper images), these values will change as reported by \citet{Bottrell2019}; however, the distributions could slightly change on the maximums.}

\section{Comparing}

{\color{red}   DS18), where classifications for about 670 000 objects from the SDSS DR7 Main Galaxy Sam- ple of Meert et al. 2015 are provided. Since about 15 per cent of the MaNGA DR15 galaxies were not included in that analysi
training a Con- volutional Neural Network 
accuracy, completeness, and contamination, should be comparable to the results in DS18 (>90 per cent for all tasks)
DL models trained with the Nair & Abraham (2010) catalogue: a TType value, a finer separation be- tween S0 and pure ellipticals (E), and the probability of having a bar feature.
The typical error in TType is ∼1.1. See fig. 13 of DS18 for a better understanding of the TType values presented in this catalogue, as well as for PS0 (which is only meaningful for ‘early-type’ galaxies, ETGs, i.e. when TType ≤ 0)
we changed TType for less than 3 per cent of the objects, and modi- fied PS0 for about 5 per cent of the objects with TType ≤ 0. Most misclassifications are due to incorrect radius values (used for the cutout size), faint galaxies, or contamination by nearby objects.
as suggested by DS18). Specifically, we use them to define two classes of LTGs: those with TType >3, and others with 0 < TType <3; objects having TType <0 and PS0 ≥ 0.5 are defined to be S0; and ellipticals (E) have TType < 0 and PS0 < 0.5. Fig. 14 in DS18 shows that essentially all Es have PS0 < 0.5, so it is very unlikely that our sample of S0s
is contaminated by Es. On the other hand, fig. 12 in DS18 shows that while TType=0 is a reasonable choice for separating S0s from other LTGs, the actual boundary is not particularly sharp. By setting the threshold at TType=0, objects we classify as LTGs may be contaminated by S0s, more than vice versa
The performance of our model is excellent for the intermediate T-types. However, it shows some flattening at the edges (see Fig. 11). For T-type > 6 that is obviously due to insufficient statistics. 
Given that we have enough ETGs to provide a more accurate classification, we train an additional model to separate E from S0 galaxies
The model output is PS0, i.e. the probability of being S0 rather than E
 only 6 per cent of the test sample with T-type = −5 in N10 is assigned PS0 > 0.5. Most of the S0/a are also correctly assigned a high PS0 , although there is a 10 per cent of them for which PS0 < 0.5}

 \subsection{Morphology and Structure in the Star Formation Main Sequence Diagram}

The Star Formation Main Sequence (hereafter SFMS) is a useful correlation to classify galaxies in terms of their Star Formation Rate and Stellar Mass ($M_{*}$), and has been recognized as a fundamental tool to understand galaxy evolution and the quenching processes \citep{Renzini2015}. Galaxies in this diagram can be classified as either Star-Forming (SFG; on the Main Sequence), Starburst galaxies (above the Main Sequence), red sequence galaxies (RSG; below the Main Sequence) and Green Valley galaxies (between the main sequence and the red sequence).


{\color{magenta} Many previous SFMS studies were carried out using integrated
quantities, however IFS surveys have allowed us to start researching the spatially resolved counterpart of the SFMS (citar los articulos relevantes, en la introduccion de mi articulo del 2019 hay una lista bastante completa de ellos).} This has been of crucial relevance to understand how the interrelation of star formation, stellar masses, and secular processes establish the physical origins and drive the observed global star-formation scaling relations. 

Recent studies have explored the dependencies of the SFMS on other galaxy properties like morphology, color or environment \citep{Popesso2019,Goddard2017,CanoDiaz2019}. A series of works propose that the slope of the SFMS and its scatter are due to an increasing prominence of a bulge coexisting with an actively star forming disk at increasing stellar masses {\color{magenta}esta frase no se entiende bien, la verdad no comprendi lo que quieren decir} (Wuyts et al. 2011, Whitaker et al. 2015, Abramson et al. 2014, Erfanianfar et al. 2016, \citealt{Morselli2017}).

\citet{Popesso2019} studied the slope of the Main Sequence SFMS of local star forming galaxies at stellar masses larger than $10^{10} M_{\odot}$ exploring the origin of its bending {\color{magenta} cual bending?} and the increase of its scatter at high stellar masses. For the SFMS bending they argue about two intervening processes: i) the formation of a bulge component as a consequence of the increased merger activity in groups, and ii) the cold gas starvation induced by the hot halo environment, which cuts off the gas inflow onto the disk. They also explain the increase of the SFMS scatter at high stellar masses as caused by the larger spread of star formation histories of central group and cluster galaxies with respect to lower mass systems. {\color{magenta} Me parece que este parrafo esta muy largo y pareciera que esta volando. Creo que es mejor mencionar estas cosas una vez que hayan presentado la figura 16 para ayudar a interpretarla}

{\color{magenta}Without trying to be exhaustive, we present a first insight into the morphological and structural behavior of MaNGA galaxies in the SFMS diagram, that may complement previous results reported recently \citep[see for example:][]{CanoDiaz2019}. For this purpose we use our homogeneous morphological evaluation for the DR15 MaNGA sample, along with carefully determined structural properties of galaxies, resulting from a 2D parametric decomposition for the same sample, given by \citetalias{Fischer2019}}

Figure~\ref{fig:mass_sfr} (upper panel) shows the SFMS diagram color-coded in terms of the morphological classification reported here. Likewise, the lower panel shows the SFMS diagram color-coded in terms of the bulge-to-total light ratio compiled from 2D decomposition by \citetalias{Fischer2019}. The fits and associated 1$\sigma$ dispersion to the Main Sequence (solid blue line) and Red Galaxies (solid red line) are taken from Table 1 of \citet{CanoDiaz2019}. 

{\color{cyan} For this section, we have exclude galaxies with inclinations $i>60^o$, since at high inclinations the derivation of the spatially resolved properties may be severely affected \citep{IbarraMedel2019}, }{\color{magenta}and to be consistent with the fits from \citet{CanoDiaz2019}}  

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/mass_sfr.png}
 \caption{Stellar mass vs SFR as a function of Hubble type (top) and B/T (bottom). Lines are the best fits for the SFMS and RS in \citet{CanoDiaz2019}. Black-open stars show the AGNs. For this plot we have discarded ancillary and highly inclined (i$>$60) galaxies. {\color{blue} Aldo: Sugeriria tambien usar isocontornos.} {\color{red} Las SFR y el ajuste de la MS es lo hecho por Mariana para galaxias con inc<70.}}
 \label{fig:mass_sfr}
\end{figure}


\citet{CanoDiaz2019} have shown that a cut at EW(H$\alpha$)= 6 $\AA$ in the central regions of galaxies {\color{magenta}En mi articulo no hago el analisis en la region central. Para las relaciones globales uso todo el FOV de MaNGA} provides a cleaner distinction between the SFMS and RGs than that produced in the Color-Magnitude Diagram (CMD). We take advantage of these results and identify galaxies into four regions of the SFMS diagram in Figure~\ref{fig:mass_sfr}. 1. Starburst galaxies as those located above the upper 1-$\sigma$ limit of the fit to the main sequence. 2. Main sequence galaxies as those located within $\pm 1-\sigma$ of the fit to the main sequence. 3. Red sequence galaxies as those located within $\pm 1-\sigma$ of the fit to the red sequence. 4. Green valley galaxies as those galaxies located in the middle region below 1-$\sigma$ of the main sequence fit and above 1-$\sigma$ of the red sequence fit \citep[c.f.][]{Sanchez2018}.


\begin{figure}
 \includegraphics[width=\columnwidth]{figures/resid_morpho.png}
 \caption{Residuals (logMass-mean[MassBin]). }
 \label{fig:residuals}
\end{figure}


\begin{figure}
 \includegraphics[width=\columnwidth]{figures/Resid_morpho2D_mean.png}
 \caption{Residuals (logMass-mean[MassBin]). }
 \label{fig:residuals2D}
\end{figure}



Figure~\ref{fig:hmorpho_mass_sfr} shows the morphological volume-corrected distribution (upper panel) and the corresponding B/T volume-corrected distribution (lower panel) of galaxies in the Starbursts, SFMS, RG and Green Valley regions by considering the best fits to the SFMS diagram in \citet{CanoDiaz2019}. Notice that here we have omitted highly inclined galaxies (i > 60) from our original sample {\color{magenta}Eso ya lo mencionaron antes, no creo que sea necesario repetirlo}.


\begin{figure}
 \includegraphics[width=\columnwidth]{figures/hist_morphoSFMSVC.png}
 \caption{Upper panel: Morphology distribution for galaxies in the Starburst (purple dashed), SFMS (solid blue), RG (solid red) and Green Valley (green dashed), normalised to the total number in each sample. Lower panel: The corresponding B/T distribution using same line symbols and colors. Highly inclined i<60 galaxies were omitted from the original sample. These distribution are volume-corrected. {\color{blue} Aldo: Igual que en las figuras anteriores sobre $n$ y $N_T$}}
 \label{fig:hmorpho_mass_sfr}
\end{figure}

From 2722 MaNGA DR15 galaxies represented the SFMS diagram, and according to our definitions, Starbursts and Main sequence galaxies account to $\sim$ 34.7\%, Green Valley galaxies $\sim$ 45.3\% and Red sequence galaxies (considering galaxies below its 1-$\sigma$ fit) $\sim$ 20\%. Notice that these fractions refer to the MaNGA sample with no volume corrections.  
{\color{cyan} Considering volume corrections percentages are, starburst and star forming $\sim$48.6\%, green valley $\sim$39.5 and Red sequence galaxies (considering galaxies below its 1-$\sigma$ fit) $\sim$ 11.9\%}

Starbursts and Main Sequence galaxies are present in practically all morphological types, most from Sa to Sd types with fractions (81.4\%) and (86.2\%) respectively, and a small fraction in very early types (c.f. Thomas et al. 2010; Gomes et al. 2016a; Lacerna et al. 2016). In contrast, the red sequence is mostly represented by early type galaxies from E to Sa types (93.5\%) with a sharp cut (no galaxies) from Sc types and later. Likewise, Green Valley galaxies show a wide morphological diversity, most from E to Sd types (99.3\%) with a sharp cut at Sdm types and later.  
{\color{cyan} For the volume-corrected sample, Starbursts and Main Sequence galaxies, from Sa to Sd types have fractions (75.5\%) and (84\%) respectively. Red Sequence, from E to Sa types (89\%). Green valley, from E to Sd types (95.4\%).}

More recently, \citet{CanoDiaz2019} examined the global and local SFMS diagrams exploring their dependence with morphology in the MaNGA MPL5 sample. Notice however, that they classified sources on a physical basis by the dominant ionizing processes; as star forming galaxies, Red/passive galaxies and those with uncertain ionization processes. However, in general they find that the morphological distribution of the star forming galaxies is populated mainly by late-type galaxies, while red galaxies present a broader morphological distribution, with a non-negligible fraction of them being early-type spirals, in qualitative agreement with our results. The morphological results presented here are also in qualitative agreement with other previous studies (e.g. Weinmann et al. 2006; James et al. 2008; Schawinski et al. 2014; Casado et al. 2015; \citealt{GonzalezDelgado2016}).


Regarding the structural content of MaNGA galaxies in distinct regions of SFMS diagram, we consider disk-dominated galaxies as those with (0 < B/T < 0.2), intermediate B/T galaxies as those with (0.2 < B/T < 0.65) and bulge-dominated galaxies as those with (0.65 < B/T < 1.0). From 2865 MaNGA MPL7 galaxies (omitting highly inclined and ancillary galaxies), 22.13\% are disk-dominated, 48.06\% are of intermediate types and 29.8\% are bulge-dominated galaxies.  
{\color{cyan} For the volume corrected sample, 26\% are disk-dominated, 59.4\% are of intermediate types and 14.6\% are bulge-dominated galaxies}

In Figure~\ref{fig:hmorpho_mass_sfr} (lower panel) starburts/SFMS, Red galaxies and Green Valley galaxies show a kind of complementary distributions among them, with starburst/SFMS showing a monothonic decreasing fraction towards high B/T values, Red sequence galaxies showing a monothonic decreasing fraction towards low B/T values and Green Valley galaxies showing a structural content in between these two extremes, all having a common intersecting region at B/T $\sim$ 0.45. {\color{red} quiza 0.4?}

Starbursts and main sequence galaxies have an important fraction of disk-dominated galaxies (0 < B/T < 0.2) (33\%) and (45\%). At the same time they show slightly different distributions mainly at intermediate B/T values (0.2 < B/T < 0.65) (58.2\%) and (48.2\%) respectively. Galaxies in SFMS are composed from pure disks to the bulk of the star forming galaxy population.
Red sequence galaxies show in contrast, an important fraction of bulge-dominated galaxies (0.65 < B/T < 1.0) (60\%).
The structural content in the Green Valley is wide with important contributions along the whole B/T interval, with relative fractions of disk-dominated (17.6\%), bulge-dominated (31.9\%) and intermediate B/T values (50.5\%).

{\color{red} Este es el mismo parrafo anterior usando la muestra corregida por volumen: }

{\color{cyan} Starbursts and main sequence galaxies have an important fraction of disk-dominated galaxies (0 < B/T < 0.2) (25.5\%) and (33.6\%). At the same time they show slightly different distributions mainly at intermediate B/T values (0.2 < B/T < 0.65) (66.3\%) and (61.9\%) respectively. Galaxies in SFMS are composed from pure disks to the bulk of the star forming galaxy population.
Red sequence galaxies show in contrast, an important fraction of bulge-dominated galaxies (0.65 < B/T < 1.0) (45.8\%).
The structural content in the Green Valley is wide with important contributions along the whole B/T interval, with relative fractions of disk-dominated (27.9\%), bulge-dominated (16.5\%) and intermediate B/T values (55.6\%).}

As already posed in Section (), MaNGA galaxies show a wide structural diversity that requires ab-initio a careful determination of B/T ratios with 2D methods as recently reported by \citetalias{Fischer2019}. This is important for the interpretation and recognition of any B/T trend along the SFMS as those studied by \citet{Morselli2018} and references therein.


%%%%% AGNS

\section{Active Galactic Nuclei}

{\color{magenta} The MaNGA survey offers the possibility to study the properties of nuclear super-massive black holes in galaxies and their relations with global properties of their hosts, such as morphology, SFR, stellar mass, etc. But also to spatially resolved properties derived from IFU observations.}   

The main criteria to identify the actual sample of AGNs in the MaNGA sample is described in (\citet{Sanchez2018}). The selection is based on the spectroscopic properties of the ionized gas in the central region (3$\times$3 arcsec) of the galaxies by imposing a double criterion; (i) that they have emission line ratios above the Kewley demarcation line (excluding star-forming regions) in three BPT diagrams and (ii) with EW($H\alpha$) larger than 1.5 $\AA$ in the central regions, following \citet{CidFernandes2010}. The final sample amounts to 243 AGNs out of 4614 galaxies ($\sim$ 5\%), similar to the fraction reported by \citet{Schawinski2010} considering only narrow line AGNs.  

{\color{red} Tenemos que quitar este parrafo:

The selection of Type-I AGNs is based on the presence of a broad (FWHM $\sim$1000-10000 km s$^{-1}$) component in the H$\alpha$ permitted line (e.g. Peterson et al. 2004, Cortes-Suarez in preparation). From 246 AGN candidates, 31 were classified as Type-I AGNs and the remaining (215) were classified as Type-II AGNs. Notice that (i) this selection is biased towards gas rich, bright nuclear sources, as other optically selected AGN samples, and that (ii) this selection criterion is different from those in other studies using MaNGA data (c.f. Rembold et al.  2018).}

Table~\ref{tab:agn} summarises the morphological distribution of 243 AGNs found in the original MaNGA (DR15) sample following the method proposed by \cite{Sanchez2018}. Columns 2 reports the fractions respect to the total number of AGNs and column 4 the fraction expected after applying the volume correction and discarding the ancillary galaxies.
 
 
\begin{table}
  \begin{center}
    \caption{Fractions of galaxies with AGNs as a function of morphology}
    \label{tab:agn}
    \begin{tabular}{c c c c}
      \hline
      \multicolumn{4}{c|}{Total of AGNs: 243} \\  
      \hline      
      \textbf{Type} & \textbf{N} & \textbf{Fraction} & \textbf{Volume-corr} \\
                    &            &                   & \textbf{fraction} \\
      \hline
E & 34 & 0.14 & 0.1 \\
S0 & 41 & 0.17 & 0.24 \\
S0a & 28 & 0.12 & 0.1 \\
Sa & 30 & 0.12 & 0.11 \\
Sab & 35 & 0.14 & 0.14 \\
Sb & 39 & 0.16 & 0.2 \\
Sbc & 19 & 0.08 & 0.05 \\
Sc & 14 & 0.06 & 0.06 \\
Scd & 3 & 0.01 & 0.01 \\
Sd & 0 & 0.0 & 0.0 \\
Sdm & 0 & 0.0 & 0.0 \\
Sm & 0 & 0.0 & 0.0 \\    
      \hline      
    \end{tabular}
  \end{center}
\end{table}

Figure~\ref{fig:agn_hist} shows on the top panel, the morphological distribution (volume-corrected) of the AGN hosts (Type-II and Type-I; red line), compared to that of their non-active counterparts (black line). Likewise and using the same symbols and colours, the bottom panel shows the stellar mass distribution (volume-corrected) of the AGN hosts (Type-II and Type-I), compared to that of their non-active counterparts.


\begin{figure}
 \includegraphics[width=\columnwidth]{figures/hist_AGNVC.png}
 \caption{Top panel: AGN (non-AGN) histogram as a function of morphology in red (black) line normalised by the total number of AGNs (non-AGNs). Bottom panel: AGN and non-AGN as a function of stellar mass, with same colour code. These distributions are volume-corrected and omitting ancillary galaxies. }
 \label{fig:agn_hist}
\end{figure}
 

AGNs are located in a range of morphological types from E to Sc galaxies. At the range Sbc-Sc, AGNs appear less frequently than their non-active counterparts, indicating no preference for optically select AGNs to be hosted in these types. In contrast, AGNs do show a significant preference to be located more in hosts from early E to intermediate Sb types (88\%) than non-active AGNs (53\%). At the late types extreme, notice the striking absence of AGNs for galaxies of types later than Sc.

{\color{red} Tenemos que quitar este parrafo:

 When considering individual I and II AGN types, at the extremes of the morphological distribution, there is no clear preference of any AGN type to be hosted either by (E) or (Sc) types, perhaps a slight preference of type I AGNs to be located more in Es than non-AGNs. Although Type-I AGNs are also found in early-type spirals, a factor of two more preference is found (54\%) for type II AGNs to be hosted from S0 to Sbc types, compared to type I AGNs (26\%).}

{\color{red}Falta revisar este trabajo:  A similar result was previously re-ported (e.g., Catalán-Torrecilla et al. 2017).}

{\color{red} \citet{CatalanTorrecilla2017} found Type-II AGNs are preferentially distributed between Sa-Sbc hosts galaxies in the CALIFA survey. }

In terms of stellar mass, AGNs are hosted in galaxies in the mass range 9.0 $< \log M_\ast/M_\odot <$ 11.5.

AGNs show a mass distribution skewed toward larger masses (average (AGN)= 10.24) compared to that of non-active galaxies (average (no-AGN) = 9.44). A Kruskal-Wallis H test confirm this with high significance (p$\sim$0) {\color{red} pendiente. 

El siguiente parrafo habria que quitarlo:

Notice that part of this skewness is driven by type I AGNs that prefer to inhabit more massive galaxies (median (AGN I) = 10.65), compared to type II AGNs (median (AGN II) = 10.42). This is also confirmed with high significance p=0.012. Type-I AGNs thus present a more strongly skewed distribution toward larger masses compared to the distribution of non-active galaxies.} 

These results are consistent with previous findings in \citet{Sanchez2018} for the MaNGA DR14 sample establishing that AGN hosts are, on average, more massive, more compact, more centrally peaked and more pressure-supported systems.
 
 
 %%%%%%% Extra Plots %%%%%
 
 
\begin{figure}
 \includegraphics[width=\columnwidth]{figures/CAS_class_nsa.png}
 \caption{CAS con datos del NSA}
 \label{fig:CAS_nsa}
\end{figure}




Figure~\ref{fig:mass_morpho2D} shows a contour-plot representation of the Hubble type distribution in terms of the original (top) and volume-corrected (bottom; with $\log (M_{\ast}/M_{\odot}) >$8.5) stellar mass. Contours were interpolated considering 12 bins corresponding to all Hubble types and then smoothed applying a $\log_{10}$ transformation to the number of galaxies in each 2D bin, so the 2D distribution decays slowly. Colour-bar is in $\log_{10}$ units. The corresponding stellar mass histogram (top panels) and Hubble type distribution (vertical-right panels) are also presented in $\log_{10}$ units.

Figure~\ref{fig:mass_morpho2D} let us appreciate a clear bi-modality in the morphological mix of the MaNGA sample; i) an early type region (E-S0a) showing a wide distribution in mass peaking at $\log(M_{\ast}/M_{\odot}) \sim$ 10, with a samll concentration of low-mass early-type galaxies and ii) the complement intermediate and late types (Sa-Sdm), with a wide mass distribution, concentrated at $\log(M_{\ast}/M_{\odot}) \sim$ 9 and another small concentration of low-mass late-type spirals.

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/mass_class2D.png}
 \caption{2D histogram of the Hubble type vs stellar mass (volume-corrected and omitting ancillary galaxies). Contour and density colours are in $\log_{10}$ units. Top panels: stellar mass distribution, and vertical-right panels: the Hubble type distribution. Note only galaxies with $\log (M_{\ast}/M_{\odot}) >$8.5 are considered. {\color{blue} Toñito: Falta describir lo que significan los numeros de la paleta para el caso sin corregir y corregido. Esto ya se aclaro en nuestras discusiones, cierto?}}
 \label{fig:mass_morpho2D}
\end{figure}


\begin{figure*}
 \includegraphics[width=0.9\textwidth]{figures/mosaics_2D.png}
 \caption{2D histograms {\color{red} Este plot es normalizado tal que la suma de todos los bines=1 solo para la parte corregida por volumen.}}
 \label{fig:mosaic2D2}
\end{figure*}

\begin{figure*}
 \includegraphics[width=0.45\textwidth]{figures/ColMas_morpho50.png}
  \includegraphics[width=0.45\textwidth]{figures/ColMas_morpho250.png}
 \caption{Colour-Mass and Morphology. {\color{red} Esta es la misma figura de arriba pero con incl<50 }}
 \label{fig:ColourMass_morpho50}
\end{figure*}

%%%%% EStadistica de barras en seccion de comparacion:

NAIR

Del catalogo de Nair en comun con nosotros MPL7 hay 1150 galaxias
 Discs in common = 937 
 Bar-Nair = 180 (180/1150)
 Bar-Nair<70 = 178  y ver quienes son las 2 restantes
 Bar-nosotros=513  (513/1150)
 Bar-nosotros<70=475 y ver quienes son las restantes (513-475)
 Bar-Nair-nosotros<70=174   en comun; ver que paso con las 6 restantes 
 porque tienen barra para Nair?
 Tipos de barra:
 Bar-Nair-nosotrosFuerte<70=146 (de 174 en comun nosotros vemos 159 fuertes (AB\_ y B))
 Bar-Nair-strong<70=15
 Bar-Nair-intermediate<70=92
 Bar-Nair-weak<70=67
 
 Bar-Nair-strong-nosotrosFuerte<70=14
 Bar-Nair-intermediate-nosotrosFuerte<70=86
 Bar-Nair-weak-nosotrosFuerte<70=46
 Bar-Nair-strong-nosotrosDebil<70=1
 Bar-Nair-intermediate-nosotrosDebil<70=6
 Bar-Nair-weak-nosotrosDebil<70=21
 
 Bar-nosotros-Nobar-Nair<70=300
 Bar-nosotros-estrucN <70=18
 
 
 GALAXY ZOO
 
 Galaxy Zoo in common 4219 galaxies
Discs in common = 3443
BarGZ = 680
BarGZstrong = 367
BarGZweak = 313
BarNosotros<70 = 1429
BarNosotrosFuerte<70 = 797
BarNosotrosDebil<70 = 632
En comun: BarGZ - BarNosotros = 631
BarGZ - BarNosotrosFuerte = 451
BarGZstrong - BarNosotrosFuerte = 319
BarGZweak - BarNosotrosFuerte = 132
BarGZstrong - BarNosotrosDebil = 46
BarGZweak - BarNosotrosDebil = 134

  \begin{figure*}
 \includegraphics[width=0.7\textwidth]{figures/Bfrac_class.png}
 \caption{Upper panels: Normalised histograms of barred galaxies (volume-corrected) as a function of stellar mass (left) and colour (right). Lower panels: fractions as a function of stellar mass (left) and colour (right). For fractions, given a bin, the number of galaxies with bar is divided by the total number of galaxies in the bin. Black lines present all bar families altogether. S0-Sb morphologies are presented in dotted-dashed-red, and Sbc-Irr in dotted-blue. {\color{blue} Aldo: Como discutimos, la simbologia de las figuras es confusa. Yo decia usar $N_T(\geq S0,\geq 10^{9}M_{\odot})$. No queda claro quien es $N$ ni $n$.}}
 \label{fig:Bfrac_class}
\end{figure*}



\section{residuals}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/Resid_colour2D_mean.png}
 \caption{Residuals (g-i - RedSeq). {\color{red} Respecto a los promedios en la secuencia roja}}
 \label{fig:residuals2D}
\end{figure}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/Resid_sfr2D_mean.png}
 \caption{Residuals (logMass-mean[MassBin]). }
 \label{fig:residuals}
\end{figure}


\begin{figure}
 \includegraphics[width=\columnwidth]{figures/Resid_age2D_mean.png}
 \caption{Residuals (Age - mean). }
 \label{fig:residualsAge}
\end{figure}

\section{Tides}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/manga-tides-comp.png}
 \caption{Galaxies with tidal debris in common with \citet{Nair2010}. Top: Galaxy with shells, middle: galaxy with tails (and bridge), and bottom: close pair with tides. Note, although we do not classify the tidal debris according to their appearance, we we detect the same structures reported in Nair.}
 \label{fig:tides_comp}
\end{figure}

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/frac_class_tidesVC.png}
 \caption{The morphological fraction (top panel) and the stellar mass fraction (bottom panel) of galaxies with tidal debris, for the original (dotted) and volume-corrected (solid) samples. The sample with tidal debris is divided into early (red) and late (blue) types. }
 \label{fig:tides_morpho}
\end{figure}



\section{MaNGA Edge-on Galaxies}
\label{sec:edgeon}

The advent of recent IFU surveys (c.f. \cite{Sanchez2012}) have shown the potential that highly inclined galaxies offer for the analysis of properties in disk galaxies including their structure, kinematics, and stellar content (c.f. Levy et al. 2019 arXiv:1905.05196v1; Jones et al. 2017; Bizyaev et al. 2017, Ho et al. 2016, L\'opez-Cob\'a et al.
2019).

Edge-on galaxies were identified as those having 
inclination $>$60$^{\circ}$ based on semi-axis b/a ratio estimates reported in \citetalias{Fischer2019} for the MaNGA DR15 sample. Notice that the morphological assignation of these systems is intrinsically tentative, and based on the procedures described in section ().

We identified 1243 highly-inclined galaxies implying 33\% of all the disks in the first half of the MaNGA sample. Figure~\ref{fig:inc_morpho} (left panel) shows the distribution of highly-inclined galaxies per morphological type bin. Likewise, the right hand panel shows the corresponding distribution per stellar mass bin. The bins are normalized to the total number of inclined galaxies.   

\begin{figure}
 \includegraphics[width=\columnwidth]{figures/hist_class_inc.png}
 \caption{The distribution of highly-inclined galaxies (>60$^o$) per 
 morphological type bin, normalized to the total number (1243) of highly 
 inclined galaxies.}
 \label{fig:inc_morpho}
\end{figure}

Edge-on galaxies are present all along the MaNGA morphological mix from S0 up to Sd types. Most of them (82.5\%) in the (Sa-Sc) range, with a strong decrease at the extremes of the distribution; (11.2\%) and (5.5\%) in the ranges (S0-S0a) and (Scd-Sd) respectively. In terms of stellar mass, Edge-on galaxies lie in the mass range 8.5 < log M(Mo) < 11.5 showing a Gaussian distribution peaked at logM $\sim$ 10. 


